Beyond Geometry: Comparing the Temporal Structure of Computation in Neural Circuits with Dynamical Similarity Analysis

How can we tell whether two neural networks utilize the same internal processes for a particular computation? This question is pertinent for multiple subfields of neuroscience and machine learning, including neuroAI, mechanistic interpretability, and brain-machine interfaces. Standard approaches for comparing neural networks focus on the spatial geometry of latent states. Yet in recurrent networks, computations are implemented at the level of dynamics, and two networks performing the same computation with equivalent dynamics need not exhibit the same geometry. To bridge this gap, we introduce a novel similarity metric that compares two systems at the level of their dynamics, called Dynamical Similarity Analysis (DSA). Our method incorporates two components: Using recent advances in data-driven dynamical systems theory, we learn a high-dimensional linear system that accurately captures core features of the original nonlinear dynamics. Next, we compare different systems passed through this embedding using a novel extension of Procrustes Analysis that accounts for how vector fields change under orthogonal transformation. In four case studies, we demonstrate that our method disentangles conjugate and non-conjugate recurrent neural networks (RNNs), while geometric methods fall short. We additionally show that our method can distinguish learning rules in an unsupervised manner. Our method opens the door to comparative analyses of the essential temporal structure of computation in neural circuits.

==> neurips/bifurcation.tex <==
\subsection{\method can detect bifurcations and large-scale reorganizations in dynamics}

In dynamical systems theory, a bifurcation occurs when the fixed point structure of the system qualitatively changes as a result of a parameter or set of parameters passing some particular threshold (\cite{strogatz_nonlinear_2015}). This can be done in a variety of ways: a stable fixed point can bifurcate into two symmetric fixed points separated by an unstable fixed point (a Pitchfork bifurcation), a fixed point can bifurcate into a limit cycle (a Hopf Bifurcation), and more. Discovering how a recurrent neural network bifurcates across training or contexts can provide characteristic insight into how and what the network learns. Importantly, this is an interesting feature of biological and artificial circuits, as well as dynamical systems in general.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{neurips/neurips4.png}
    \caption{\method detects bifurcations and bit flip onsets, identifies qualitative differences in RNN architecture training dynamics. \textbf{a.} Schematic of the delayed-bit onset task hidden states in 3 PC's. \textbf{b.}  Averaged stepwise comparison of RNN dynamics across training (blue, epoch t vs t+30) and corresponding number of fixed points (yellow). Shading indicates standard error.\textbf{c.} Pairwise similarities across training for each RNN architecture. White dotted lines demonstrate the times at which a new bit was introduced in the task.}
    \label{fig:bifurcation}
\end{figure}

We applied \method to hidden states from the same RNN pairwise across training in a modified version of the 3-bit FlipFlop task, in which we introduced new bits to the task iteratively across training (at 0, 300, and 600 epochs respectively). A visual depiction of the iterative bifurcation in the dynamics is shown in Fig. \ref{fig:bifurcation}a. In Fig. \ref{fig:bifurcation}b, we display the results of applying \method between epochs $t$ and $t+30$ iteratively across training, averaged over 58 networks of different architectures, and DMDs of different number of delays and ranks. \method is able to clearly identify the onset of a new bit, as evidenced by the clear peaks in the dissimilarity. Likewise, the dissimilarity remains high for the next few timesteps, which is when the bifurcation occurs--this is displayed by the rapid jumps in the number of stable fixed points (yellow curve). Importantly, the first peak of dissimilarity perfectly aligns to the epochs in which the first bifurcation occurs (between epoch 30 and 120), suggesting that the \method is picking up the signal of the bifurcation.  

Next, we utilized \method to identify qualitative differences in learning dynamics across different RNN architectures. We applied \method to each type of RNN architecture with a DMD of rank 50 and 50 delays between each timepoint in the dynamics and plotted the dissimilarity as heatmaps in \ref{fig:bifurcation}c. From these plots, we are able to identify that these networks learn the task in two ways: In the first, represented by the Vanilla RNN and the LSTM, learning appears to occur uniformly bit-by-bit, with only small changes occurring within a single bit's interval. In the second, represented by both types of gated networks, the network undergoes a sharp change in the middle of the first bit-interval, and progressively slows down from there. For all architectures, the later bit onsets induce smaller changes, and each stage of training is evident from the block-like structure of the heatmaps.


==> neurips/changing_topology.tex <==



==> neurips/extra_neurips.tex <==
\subsection{Extra DMD}
Originally developed in the fluid dynamics community, the goal of the DMD is to identify spatiotemporal coherent structures of the underlying high-dimensional dynamical system. This approach is distinct from standard methods like Principal Components Analysis (PCA) which only seeks to identify spatially coherent structures, or the Fourier Transform and its siblings like the Wavelet Transform, which only seek to identify temporally coherent structure. 

The matrix $A$ can then be decomposed into its eigenvalues and eigenvectors, which are called the \textit{dynamic modes} of the system. The eigenvalues therefore describe decay rates and frequencies for the system dynamics along their respective modes.  One of the main issues with appropriately identifying a finite linear representation of nonlinear dynamics is identifying the measurement subspace, which must be closed under the operation of $A$. A variety of methods abound, including extended and kernel DMD (which introduce polynomial observables into X). 

 Recent methods in computational neuroscience such as the Switching Linear Dynamical Systems seek to model a nonlinear system as a set of linear systems defined by attractor basins, where the switching between basins is fit to the system via a Hidden Markov Model \cite{linderman_recurrent_2016}. However, these models are complex to implement and fail to provide a unified view of the system in light of its local parts. 

 Beyond capturing temporal information, DMRSA has multiple advantages over standard methods. 
\subsection{Extra methods}

Because the DMD identifies dimensions in the space of data that are both spatially and temporally coherent, this comparison can be viewed as both comparing the geometric relationships between dynamic modes in each system and comparing their dynamical properties, such as whether the modes grow, shrink, or oscillate. Beyond capturing temporal information, DMRSA has multiple advantages over standard methods. The DMRSA simply integrates noisy trials into its estimate. Unlike spatial shape analyses, which require averaging over multiple noisy trials in the same condition to arrive at one 'representation' of each condition-time point, DMRSA utilizes each of these trials in its estimate of neural dynamics. The importance of these noise perturbations in estimating dynamics has been highlighted in \cite{galgali_residual_2023} Thus, DMRSA takes full advantages of all trials available. 

Note that because of this operation, DMRSA has the flexibility to work with multiple conditions and multiple trials, a single condition with multiple trials, or even a single trial alone. It is worth noting that utilizing multiple conditions, which are defined by different input stimuli, can alter the structure of the Dynamic Mode matrix, but this may help the system better capture purely recurrent dynamics by forcing the regression to average over unseen input.

The Hankel tensors will be partially flattened into the shape $H_x \in \mathbb{R}^{ck(t-p-1) \times op}$. We decompose these matrices via Singular Value Decomposition: $H_x = U_x S_x V_x^T$, where $U_xS_x$ describe the basis of the data, and $V_x$ are the so-called eigen-time delay coordinates, describing the behavior of the system in the basis. Likewise, $H_x'$ is decomposed as $H_x' = U_xS_xV_x'^T$ in the same basis, with only the time delay coordinates shifted. Next, we fit a reduced-rank regression model to the eigen-time delay coordinates to arrive at Dynamic Mode matrices $A_x, A_y \in \mathbb{R}^{op \times op}$. Note that we are agnostic to form of the regression model. It may be applied as a sparse regression model (as in the Sparse Identification of Nonlinear Dynamics, \cite{brunton_discovering_2016}), a penalized regression, a low-rank regression, or any other generic form. In this paper, we opted for a low-rank, L2-penalized regression. Finally, we directly apply a shape analysis metric to our two dynamic mode matrices, thereby treating $A_x, A_y$ as our new data. 


\section{Extra Results}
Although our method was successful at identifying the dynamical structure in RNNs trained to perform the 3-bit flip-flop task, the dynamics in this task observed in data are mostly static, as activity tends to concentrate around the fixed points. Thus, we wanted to further validate our method on a task that required a dynamic representation, in that neural activity needs to continuously move within its state space. We chose to use the Sine Wave Task as trained RNNs utilize limit cycles in their hidden state to solve this task. For details on this task, see \cite{maheswaranathan_universality_2019}. For brevity, we only display the key result: the comparison of our method to the standard spatial shape analysis in comparing network representations across architectures (Figure \ref{sinewave}). Here, we used SVCCA \cite{raghu_svcca_2017} as our similarity metric. To compute the DMRSA, we projected neural activity down to 10 dimensions using PCA and then embedded the trajectories into the Hankel matrix using a lag of 50. We sampled 320 trials of 150 time steps each, and fit our HAVOK matrix with a rank of 20 (400 parameters total). Details describing the HAVOK model's fit to data are in the supplementary figures. There, we additionally show MDS embeddings using other similarity metrics (Procrustes and CKA). As in Figure \ref{flipflop}, models intermingle across architectures in the DMRSA metric space, indicating that the DMD has captured universal dynamical structure that RNNs use to solve this task. This is not the case in the standard spatial similarity analysis, which tends to focus on individualistic properties of each architecture's representational geometry. 

For the first case, we train a collection of 50-unit RNNs on tasks used in \citet{maheswaranathan_universality_2019}. Importantly, these networks have different representational geometry but equivalent attractor topology. We focus here on the well-known 3-bit Flip Flop task from \citet{sussillo_opening_2013} for the sake of space and its well-studied dynamical properties. Following \citet{maheswaranathan_universality_2019}, we tested each RNN on the same input conditions and extracted their recurrent states.

Furthermore, \citet{hart_embedding_2020} proved that a sufficiently high dimensional embedding of a nonlinear dynamical system can perfectly predict the next observation with a simple linear readout. This implies that the embedding is topologically equivalent via a \textit{linear} homeomorphism to the original system. We leverage this result in the next section to develop our similarity metric.
If these DMD matrices are fit to topologically equivalent systems (which are homeomorphic), and these matrices in turn are linearly homeomorphic to those systems according to \citet{hart_embedding_2020}, then these two DMD matrices must therefore be homeomorphic. When two linear systems are homeomorphic, this means that their dynamics matrices are similar, i.e., $A_x = CA_yC^{-1}$ for some invertible matrix C (See Supplementary Information for a commutation diagram). 

Here, alignment means that instead of fully retraining a decoder, one identifies how a neural system changes day-to-day, and applies a transformation to the decoder to account for this change. 

Previous methods also utilized neural networks (\cite{Karpowicz2022}) and the observation that neural activity in the motor cortex typically lies in a preserved low-dimensional space (\cite{gallego_cortical_2018,degenhart_stabilization_2020}) to perform alignment. As discussed above, alignment methods based on latent geometry fail to account for the underlying dynamical system and therefore may fall short of optimal alignment. We suggest that \method could be used as a direct replacement or supplement to align decoders in a BCI pipeline, as \method is more theoretically aligned with the structure of the underlying system from which BCI seeks to decode. 

%why is this better?
%By aligning the dynamics that give rise to a low-dimensional manifold, \method has the capability of abstracting away geometric perturbations to the neural manifold, which should improve decoding accuracy with limited computational cost. 
%\subsection{Identifying the brain's learning rules from dynamics}
